Bialgebraic Reasoning on Stateful Languages

Reasoning about program equivalence in imperative languages is notoriously challenging, as the presence of states (in the form of variable stores) fundamentally increases the observational power of program terms. The key desideratum for any notion of equivalence is compositionality, guaranteeing that subprograms can be safely replaced by equivalent subprograms regardless of the context. To facilitate compositionality proofs and avoid boilerplate work, one would hope to employ the abstract bialgebraic methods provided by Turi and Plotkin's powerful theory of mathematical operational semantics (a.k.a. abstract GSOS) or its recent extension by Goncharov et al. to higher-order languages. However, multiple attempts to apply abstract GSOS to stateful languages have thus failed. We propose a novel approach to the operational semantics of stateful languages based on the formal distinction between readers (terms that expect an initial input store before being executed), and writers (running terms that have already been provided with a store). In contrast to earlier work, this style of semantics is fully compatible with abstract GSOS, and we can thus leverage the existing theory to obtain coinductive reasoning techniques. We demonstrate that our approach generates non-trivial compositionality results for stateful languages with first-order and higher-order store and that it flexibly applies to program equivalences at different levels of granularity, such as trace, cost, and natural equivalence.

==> additional-macros.tex <==
%
%

\DeclareMathSymbol{\mathinvertedexclamationmark}{\mathord}{operators}{'074}
\DeclareMathSymbol{\mathexclamationmark}{\mathord}{operators}{'041}
\makeatletter
\newcommand{\raisedmathinvertedexclamationmark}{%
  \mathord{\mathpalette\raised@mathinvertedexclamationmark\relax}%
}
\newcommand{\raised@mathinvertedexclamationmark}[2]{%
  \raisebox{\depth}{$\m@th#1\mathinvertedexclamationmark$}%
}
\makeatother

\newcommand{\longTo}{\Longrightarrow}
\newcommand{\Pt}{V}
\newcommand{\R}{\mathcal{R}}
\newcommand{\st}{\mathsf{st}}
\newcommand{\lsmc}{\fatsemi}
\newcommand{\Pre}{\mathbf{Pre}}
\newcommand{\Pow}{\mathcal{P}}
\newcommand{\xTo}{\xRightarrow}
\makeatletter
\renewcommand\xRightarrow[2][]{
  \ifx\relax#1\relax%
    \ext@arrow 0055{\Rightarrowfill@}{}{#2\ }
  \else%
    \ext@arrow 0055{\Rightarrowfill@}{#1\ }{#2\ }
  \fi
}
\makeatother
\newcommand{\HJBis}{\mathbf{HJBisim}}
\newcommand{\Bis}{\mathbf{Bisim}}
\newcommand{\primrec}{\mathsf{pr}\,}
\newcommand{\hattau}{\hat{\tau}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatbeta}{\hat{\beta}}
\newcommand{\lft}{{\mathsf{l}}}
\newcommand{\rgt}{{\mathsf{r}}}
\newcommand{\colim}{\mathsf{colim}}
\newcommand{\terminal}{\mathexclamationmark}
\newcommand{\initial}{\raisedmathinvertedexclamationmark}
\newcommand{\smc}{\mathbin{;}}
\newcommand{\hatR}{{\widehat{R}}}
\newcommand{\qand}{\quad\text{and}\quad}
\newcommand{\qqand}{\qquad\text{and}\qquad}
\newcommand{\rsto}{\rightsquigarrow}
\newcommand{\pb}[2]{\scalebox{#1}{\rotatebox{#2}{$\ulcorner$}}}
\newcommand{\deq}[1]{{\rotatebox{#1}{$=$}}}
\newcommand{\dleq}[1]{{\rotatebox{#1}{$\preceq$}}}
\newcommand{\dgeq}[1]{{\rotatebox{#1}{$\succeq$}}}
\newcommand{\cev}[1]{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}
\newcommand{\diag}{\mathsf{in}}
\newcommand{\HO}{\mathcal{HO}}
\newcommand{\Refl}{\mathbf{Refl}}
\newcommand{\Gra}{\mathbf{Gra}}
\newcommand{\RGra}{\mathbf{RGra}}
\newcommand{\RRel}{\mathbf{RRel}}
\newcommand{\happrox}{\mathrel{\hat\lessapprox}}
\newcommand{\happroxs}{\mathrel{\hat\approx^{\star}}}
\newcommand{\under}[1]{\lvert#1\rvert}
\newcommand{\SKI}{\mathrm{SKI}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\ap}{{\mathrm{ap}}}
\newcommand{\var}{\mathsf{var}}
\newcommand{\cn}{{\mathrm{cn}}}
\newcommand{\cv}{{\mathrm{cv}}}
%
%
\newcommand{\Powf}{\mathcal{P}_{\omega}}
\newcommand{\FSigma}{{\mathbb{\Sigma}}}
\newcommand{\FSigmas}{{\mathbb{\Sigma}}^\star}
\newcommand{\Sigmas}{\Sigma^{\star}}
\newcommand{\FDelta}{{\mathbb{\Delta}}}
\newcommand{\FDeltas}{{\mathbb{\Delta}}^\star}
\newcommand{\ar}{\mathsf{ar}}
%
\newcommand{\NT}{\mathrm{Nat}}
\newcommand{\supp}{\mathsf{supp}}
\newcommand{\epito}{\twoheadrightarrow}
\newcommand{\abs}{\mathsf{abs}}
\newcommand{\conc}{\mathsf{conc}}
\newcommand{\T}{{\mathcal{T}}}
\renewcommand{\S}{{\mathcal{S}}}
\newcommand{\can}{\mathsf{can}}
\newcommand{\lab}{\mathsf{label}}
\newcommand{\leaves}{\mathsf{leaves}}
\newcommand{\incl}{\mathsf{in}}
\newcommand{\seq}{\subseteq}
\newcommand{\ol}{\overline}
\newcommand{\out}{\mathsf{out}}
\newcommand{\outl}{\mathsf{l}}
\newcommand{\outr}{\mathsf{r}}
\newcommand{\trc}{{\mathsf{trc}}}
\newcommand{\fn}{{\mathsf{fn}}}
\newcommand{\beh}{{\mathsf{beh}}}
\providecommand{\C}{}
\providecommand{\D}{}
\providecommand{\E}{}
\renewcommand{\C}{{\mathbb{C}}}
\renewcommand{\D}{{\mathbb{D}}}
\renewcommand{\E}{{\mathbb{E}}}
\renewcommand{\id}{{\mathsf{id}}}
\newcommand{\Nat}{\mathds{N}}
\renewcommand{\NT}{\mathsf{Nat}}

%
%
\newcommand{\stimes}[1]{{S\product #1}}
\newcommand{\xtimes}[1]{{X\product #1}}
\newcommand{\ytimes}[1]{{Y\product #1}}
\newcommand{\sbrks}[1]{{ \brks{\fst,#1}  }}
\newcommand{\cpair}[2]{{ #1, #2 }}
\newcommand{\tpair}[2]{{ #1 \product #2 }}


%
%
%
\renewcommand{\brack}[1]{\lbrack #1 \rbrack}
%
\newcommand{\sbrack}[1]{\llbracket #1 \rrbracket}
%
\newcommand{\ssbrack}[1]{\llbracket\mkern-4.7mu\llbracket #1 \rrbracket\mkern-4.7mu\rrbracket}
%
\newcommand{\f}{\oname{f}}
\newcommand{\fii}{\oname{f}}
%

%
\newcommand{\takeout}[1]{\empty}

\newcommand{\ini}{\iota}
\newcommand{\ter}{\tau}
\newcommand{\wh}{\widehat}
\DeclareMathOperator{\Coalg}{\mathsf{Coalg}}
\DeclareMathOperator{\Alg}{\mathbf{Alg}}
%
\newcommand{\cofun}{(\overline{\rule{-1pt}{7pt}\argument})}
\renewcommand{\rho}{\varrho}
\newcommand{\N}{\mathds{N}}
\newcommand{\opp}{\mathsf{op}}
\newcommand{\xla}[1]{\xleftarrow{~#1~}}
\newcommand{\mypowfin}{\mathscr{P}_\omega}

%
\newcommand{\pullbackangle}[2][]{\arrow[phantom,to path={
                     -- ($ (\tikztostart)!1cm!#2:([xshift=8cm]\tikztostart) $)
                        node[anchor=west,pos=0.0,rotate=#2,
                        inner xsep = 0]
                        {\begin{tikzpicture}[minimum
                        height=1mm,baseline=0,#1]
    \draw[-] (0,0) -- (.5em,.5em) -- (0,1em);
                        \end{tikzpicture}}}]{}}

%
%
%
%

